Thermal QCD in a non-uniform magnetic background

Off-central heavy-ion collisions are known to feature magnetic fields with magnitudes and characteristic gradients corresponding to the scale of the strong interactions. In this work, we employ equilibrium lattice simulations of the underlying theory, QCD, involving similar inhomogeneous magnetic field profiles to achieve a better understanding of this system. We simulate three flavors of dynamical staggered quarks with physical masses at a range of magnetic fields and temperatures, and extrapolate the results to the continuum limit. Analyzing the impact of the field on the quark condensate and the Polyakov loop, we find non-trivial spatial features that render the QCD medium qualitatively different as in the homogeneous setup, especially at temperatures around the transition. In addition, we construct leading-order chiral perturbation theory for the inhomogeneous background and compare its prediction to our lattice results at low temperature. Our findings will be useful to benchmark effective theories and low-energy models of QCD for a better description of peripheral heavy-ion collisions.

==> reply.tex <==
We thank the referees for their positive opinion on our work and for their constructive suggestions. Below we respond to the points raised by Referee 1.

1) The data points published in our ancillary files as well as the curves in Figs. 4-6 correspond to the local values of our observables, including statistical/systematic errors. The referee is right that there are correlations among different spatial points, so that the statistical error of differences, e.g. $\Sigma(x)-\Sigma(x')$ tend to be smaller than that of $\Sigma(x)$ itself.

To highlight this aspect, we include two figures in the lower panel of Fig. 8, where a subtraction of the condensate at the edge of the volume is performed. This makes the dip structure much more visible.

We also updated the plots in the upper panel of this figure and included one sentence describing the figure at the end of section 4. Moreover we updated the plots of figure 4 and figure 5 to show the same values of the magnetic fields.

2) The referee is right that in the heavy-ion collision setup, the magnetic field depends on not just one of the spatial coordinates. Here we only considered a one-dimensional spatial dependence instead, but our approach can be simply generalized to include more complicated spatial inhomogeneities. Another reason to consider the one-dimensional case was to enable a direct comparison to the analytically solvable setup, that can be implemented in effective models of QCD.

We included a brief discussion on this aspect in the third to the last paragraph of the introduction.

==> simulation_parameters.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c}
0.483142850731 & 3.263	& 68  & 0.020313459015	& 0.571824 & 1.19959353810 & 7.730285612	& 3	  & 0.5	  \\
0.361545320025 & 3.373	& 91  & 0.009060700472	& 0.255058 & 1.60304949228 & 5.784725120	& 5	  & 0.74 \\
0.289787520851 & 3.450	& 113 & 0.005745222025	& 0.161728 & 2	           & 4.636600334	& 6	  & 0.91 \\
0.265251415279 & 3.480	& 124 & 0.004919538188	& 0.138485 & 2.18500263643 & 4.244022644	& 6	  & 0.95 \\
0.252977532944 & 3.496	& 130 & 0.004549676793	& 0.128074 & 2.29101388948 & 4.047640527	& 7	  & 1.05 \\
0.241978505087 & 3.511	& 136 & 0.004239692720	& 0.119347 & 2.39515093083 & 3.871656081	& 7	  & 1.07 \\
0.232158344821 & 3.525	& 142 & 0.003978507993	& 0.111995 & 2.49646439437 & 3.714533517	& 7	  & 1.09 \\
0.222104425187 & 3.540	& 148 & 0.003725008881	& 0.104859 & 2.60947093339 & 3.553670803	& 8	  & 1.2	  \\
0.212524139583 & 3.555	& 155 & 0.003495506217	& 0.098399 & 2.72710216749 & 3.400386233	& 8	  & 1.22 \\
0.203409958145 & 3.570	& 162 & 0.003287147425	& 0.092533 & 2.8492953196  & 3.254559330	& 9	  & 1.33\\
0.186525967996 & 3.600  & 176 & 0.002924362345	& 0.082321 & 3.10720833097 & 2.984415488	& 9	  & 1.39 \\
0.176191575574 & 3.620	& 187 & 0.002716109072	& 0.076459 & 3.28945944103 & 2.819065209	& 10	& 1.51 \\
0.151414857544 & 3.675	& 217 & 0.002249939235	& 0.063336 & 3.82772900297 & 2.422637721	& 11	& 1.72 \\
0.132803483021 & 3.725	& 248 & 0.001927185654	& 0.054250 & 4.36415543113 & 2.124855728	& 13	& 2.02 \\
0.117278081384 & 3.775	& 280 & 0.001672198019	& 0.047072 & 4.94188713577 & 1.876449302	& 14	& 2.26 \\
0.109717277700 & 3.803	& 300 & 0.001551975837	& 0.043688 & 5.28244095929 & 1.755476443	& 15	& 2.44 \\
\end{tabular}
\caption{Caption}
\label{tab:sim_pars}
\end{table}
